FedPass: Privacy-Preserving Vertical Federated Deep Learning with Adaptive Obfuscation

Vertical federated learning (VFL) allows an active party with labeled feature to leverage auxiliary features from the passive parties to improve model performance. Concerns about the private feature and label leakage in both the training and inference phases of VFL have drawn wide research attention. In this paper, we propose a general privacy-preserving vertical federated deep learning framework called FedPass, which leverages adaptive obfuscation to protect the feature and label simultaneously. Strong privacy-preserving capabilities about private features and labels are theoretically proved (in Theorems 1 and 2). Extensive experimental result s with different datasets and network architectures also justify the superiority of FedPass against existing methods in light of its near-optimal trade-off between privacy and model performance.

==> Section/Background.tex <==
\section{Background}

\subsection{Multi-objective federated learning}

Pareto frontier...

\subsection{Attack in Federated Learning}
In this work, for our architecture, we consider all participants, including $K$ clients and the server, are \textit{honest-but-curious} adversaries. They possibly do some calculations to obtain the private data of clients by observing the model weights and updates, but they do not maliciously modify their
own inputs or parameters for the attack purpose. There are considered in our study: DLG and MI attack.\\
\textbf{DLG} Deep leakage attack is firstly proposed by \cite{zhu2020deep}, where the server tries to recover the original data based on updates and model weights. Consider $k_{th}$ client who submit its gradient $\nabla W_{pub}$ of public model. To reconstruct the raw data of client $k$, firstly initializing a dummy input $\mathbf{x}^{\prime}$ with label $\mathbf{y}^{\prime}$. Then, feeding the dummy data into the model and get the dummy gradient:

\begin{equation}
\label{dummy_grad}
\nabla W^{\prime}_{pub}=\frac{\partial \ell\left(F\left(\mathbf{x}^{\prime}, W\right), \mathbf{y}^{\prime}\right)}{\partial W}.
\end{equation}

\begin{equation}
\label{eq:dlg}
    \mathbf{x}^{\prime *}, \mathbf{y}^{\prime *}=\underset{\mathbf{x}^{\prime}, \mathbf{y}^{\prime}}{\arg \min }\left\|\nabla W_{pub}^{\prime}-\nabla W_{pub} \right\|^{2}
\end{equation}
 where $\ell$ is the classification loss, $F$ is the forward function.

By minimizing the differences between the dummy gradients and the original gradients (as shown in equation \ref{eq:dlg}), the attackers could learn a good input $\mathbf{x}^{\prime *}$ and $\mathbf{y}^{\prime *}$. In particular, DLG could easily recover the private model's output and even recover the original image if the private model is leaked, which is similar to the white-box attack.
\\\textbf{MI} However, sometimes, the attacker may not know the weights of the private model. In this case, model inversion attack (MI \cite{he2019model}) provides a strategy to reconstruct the original image. MI attack attempts to recover the original input given the private model output as the following two cases: (1) In the white-box setting, the adversary knows the private model on the participant. (2) In the black-box setting, the model parameters on the participant are unavailable for the adversary. In our setting, we mainly consider the second case. The server may conspire with the curious client to obtain other clients' data. The server provides the updated weights and gradients of the public model to reconstruct the output of the private model, and the curious client offers his own private model as the target model.

Specifically, given the private model output $O_{prt}$ and target model $F$, MI attack learns a good dummy input $\mathbf{x}^{\prime *}$ by solving the equation \ref{eq:MIA}.
\begin{equation}
\label{eq:MIA}
    \mathbf{x}^{\prime *} =\underset{\mathbf{x}^{\prime}}{\arg \min }\left\|F(\mathbf{x}^{\prime})-O_{prt}\right\|^{2}
\end{equation}

\subsection{Periodic Neurons} \label{sec:periodic neurons}
Let $\gamma = \gamma(d) >1$ be a sequence of numbers indexed by the input dimension
$d \in N$, and let $\phi: R \to [-1,1]$ be an 1-periodic function. We denote by $\mathcal{F}_\gamma^\phi$ the function class
\begin{equation}
    \mathcal{F}_\gamma^\phi = \{ f: R^d \to [-1,1] | f(x) = \phi(\gamma<w,x>), w\in S^{d-1} \} 
\end{equation}


Note that each member of the function class $\mathcal{F}_\gamma^\phi$ is fully characterized by a unit vector $w \in S^{d-1}$. We refer such function classes as periodic neurons. 

\subsection{Security Analysis of Periodic Neurons}
\subsubsection{Average-Case Decision Problems}
In the average case decision problems the statistician receives $m$ samples from either a distribution $D$ or another distribution $D_0$, and needs to decide based on the produced samples whether the generating distribution is $D$ or $D_0$. We assume that the statistician may use any, potentially randomized, algorithm $A$ which is
a measurable function of the $m$ samples and outputs the Boolean decision {YES,NO} corresponding to their prediction of whether D or D0 respectively generated the observed samples. Now, for any Boolean-valued algorithm A examining the samples, we define the advantage of $A$ solving the decision problem, as the sequence of positive numbers.
\begin{equation}
    |P_{x\in D} [\calA(x) = \text{Yes}] - P_{x\in D_0} [\calA(x) = \text{No}] |
\end{equation}

\subsubsection{Decision and Phaseless CLWE}
\begin{defi}{\textbf{Phaseless CLWE $A_{w, \beta, \gamma}$}}
We define the Phaseless-CLWE distribution on dimension d with frequency $\gamma$, $\beta-$ bounded adversarial noise, hidden direction $w$ to be the distribution of the pair $(x,z) \in \mathbb{R}^d \times [0, 1/2]$ where $x \in N(0, I_d)$ and
\begin{equation}
    z = \epsilon \gamma <w,x> + \xi \quad \text{mod} 1
\end{equation}
for some $\epsilon \in \{-1, 1\}$ such that $z \geq 0 $ and bounded noise $|\xi|< \beta$.
\end{defi}

\begin{defi}{\textbf{Decision phaseless CLWE}}. For parameters $\beta, \gamma >0 $, the average-case decision problem $\text{CLWE}_{\beta, \gamma}$ is to distinguish from i.i.d samples the following two distributions over $\mathbb{R}^d \times [0,1]$ with non-negligible advantage: 1) the Phaseless CLWE distribution $A_{w, \beta, \gamma}$ 2) $N(0, I_d) \times U[0,1]$.
\end{defi}




% \subsection{Security Analysis}
\begin{lem}  \label{lem:lemma1}
Assume $\beta \in[0, 1]$. Suppose that one receives a sample $(x, \Tilde{z})$ from the periodic neurons on dimension d with frequency $\gamma$ under $\beta$-bounded adversarial noise, and invertible periodic function $\phi: [-C, C] \to [-1, 1]$ in one single period. Let $\Bar{z} := sgn(\Tilde{z})min(1, |\Tilde{z}|)$.
Then, the pair $(x, \phi^{-1}(\Bar{z})/(2C) mod 1)$ is a sample from the Phaseless-CLWE distribution on dimension d with frequency $\gamma$ under $\frac{1}{2C}\phi^{-1}(1-\beta)$-bounded adversarial noise.
\end{lem}
According to Lemma \ref{lem:lemma1}, we could define the decision periodic neurons problem as follows:
\begin{defi}{\textbf{Decision periodic neurons}}. For parameters $\beta, \gamma >0 $, the average-case decision problem $\text{PN}_{\beta, \gamma}$ is to distinguish from i.i.d samples the following two distributions over $\mathbb{R}^d \times [0,1]$ with non-negligible advantage: 1) the Phaseless CLWE distribution $B_{w, \beta, \gamma}$ 2) $N(0, I_d) \times g(U[0,1])$, where $g: x \to \phi^{-1}(x) mod 1$.
\end{defi}

\begin{thm}
If $\phi^{-1}$ satisfies lipticiz condition, then a polynomial-time algorithm that solves \textbf{Decision phaseless CLWE} implies a polynomial-time quantum
algorithm for solving  \textbf{Decision periodic neurons}
\end{thm}

==> Section/Method.tex <==
\section{Cryptographic Security of FedPN}
\subsection{Threat model}
In this work we consider a federated deep learning scenario, where $K$ participants collaboratively learn a multi-layered deep neural network model without exposing their private training data \cite{}. We assume certain participants or the server might be \textit{semi-honest} adversary, in the sense that they do not submit any malformed messages but may launch \textit{privacy attacks} on exchanged information from other participants.

A single client has a private data $x$ and exposed public information $O$ which is related to private data by a mapping $O=g(x)$. Note that the mapping $g()$ is assumed to be \textit{known to all participants} in federated learning, while data $x$ is kept secret only to its owner. For instance, in the context of federated deep neural network learning, $O$ is the exchanged network model parameters or its gradients depending on input training data $x$. Adversaries have the following two goals
\begin{itemize}
    \item \textbf{Case 1:} Attackers don't know the weights of periodic neurons, only know weights of classifier; 
    \item \textbf{Case 2:} Attackers can observe: 1) the weights of periodic neurons; 2) the weights of classifier; 
\end{itemize}

% \subsection{The Randomness of Output for Periodic Neurons}

% \begin{lem}  \label{lem:lemma1}
% Assume $\beta \in[0, 1]$. Suppose that one receives a sample $(x, \Tilde{z})$ from the periodic neurons on dimension d with frequency $\gamma$ under $\beta$-bounded adversarial noise, and invertible periodic function $\phi: [-C, C] \to [-1, 1]$ in one single period. Let $\Bar{z} := sgn(\Tilde{z})min(1, |\Tilde{z}|)$.
% Then, the pair $(x, \phi^{-1}(\Bar{z})/(2C) mod 1)$ is a sample from the Phaseless-CLWE distribution on dimension d with frequency $\gamma$ under $\frac{1}{2C}\phi^{-1}(1-\beta)$-bounded adversarial noise.
% \end{lem}
% According to Lemma \ref{lem:lemma1}, we could define the decision periodic neurons problem as follows:
% \begin{defi}{\textbf{Decision periodic neurons}}. For parameters $\beta, \gamma >0 $, the average-case decision problem $\text{PN}_{\beta, \gamma}$ is to distinguish from i.i.d samples the following two distributions over $\mathbb{R}^d \times [0,1]$ with non-negligible advantage: 1) the Phaseless CLWE distribution $B_{w, \beta, \gamma}$ 2) $N(0, I_d) \times g(U[0,1])$, where $g: x \to \phi^{-1}(x) mod 1$.
% \end{defi}

% \begin{thm}
% If $\phi^{-1}$ satisfies lipticiz condition, then a polynomial-time algorithm that solves \textbf{Decision phaseless CLWE} implies a polynomial-time quantum
% algorithm for solving  \textbf{Decision periodic neurons}
% \end{thm}


\begin{itemize}
    \item Leverage Cos neural: 1) known model cannot infer x ; 2) $w$ and gradients is leaked, whether privacy is leaked? resist gradient leakage attack ; 3) cannot infer multiple x; 4) adding conjecture about cos neural;
    \item Analyze the cos output is largely different from x.
\end{itemize}




